LLM App Squatting and Cloning

Impersonation tactics, such as app squatting and app cloning, have posed longstanding challenges in mobile app stores, where malicious actors exploit the names and reputations of popular apps to deceive users. With the rapid growth of Large Language Model (LLM) stores like GPT Store and FlowGPT, these issues have similarly surfaced, threatening the integrity of the LLM app ecosystem. In this study, we present the first large-scale analysis of LLM app squatting and cloning using our custom-built tool, LLMappCrazy. LLMappCrazy covers 14 squatting generation techniques and integrates Levenshtein distance and BERT-based semantic analysis to detect cloning by analyzing app functional similarities. Using this tool, we generated variations of the top 1000 app names and found over 5,000 squatting apps in the dataset. Additionally, we observed 3,509 squatting apps and 9,575 cloning cases across six major platforms. After sampling, we find that 18.7% of the squatting apps and 4.9% of the cloning apps exhibited malicious behavior, including phishing, malware distribution, fake content dissemination, and aggressive ad injection.

==> Sections/related.tex <==
\section{Related work}
\label{related}


==> Tables/motivation_old.tex <==
\begin{table*}[!htbp]
    \centering
    \caption{Results of the motivating study. \xy{update}}
    \resizebox{0.6\linewidth}{!}{%
    \begin{threeparttable}
    \begin{tabular}{lrrrrrr}
        \toprule[1.2pt]
        \multirow{2}{*}{\textbf{App Name(\# of conversation)}} & 
        \multicolumn{3}{c}{\textbf{AppCrazy}} & & 
        \multicolumn{3}{c}{\textbf{LLMappCrazy}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        \textbf{\# of generated app names} & \textbf{\# of identified squatting apps} \\
        \midrule
        image generator(6M+)     & 78         & 2       & 363       & 3        \\ 
        Consensus(5M+)           & 39         & 0       & 324      & 0            \\
        Write For Me(4M+)        & 53         & 1       & 338      & 3             \\
        Logo Creator(2M+)        & 59         & 9       & 344      & 35        \\
        Canva(2M+)               & 22         & 1       & 307      & 1       \\
        Scholar GPT(2M+)         & 29         & 7       & 314      & 12        \\
        Code Copilot(2M+)        & 65         & 7       & 350      & 7         \\
        Cartoonize Yourself(2M+) & 92         & 1       & 377      & 1       \\
        Diagrams\tnote{1}(1M+)  `& 175        & 0       & 444      & 0        \\
        Python(1M+)              & 13         & 0       & 298      & 244      \\
        \midrule
        Total                    & 625        & 28     & 3459        & 274  \\
        \bottomrule[1.2pt]
    
    \end{tabular}
    \begin{tablenotes}  % 开始 tablenotes 环境，添加对应的脚注内容
        \footnotesize
        \item[1] Diagrams: The full name of this app is ``Diagrams: Show Me | charts, presentations, code''.
    \end{tablenotes}
    \end{threeparttable} }
    \label{tab:motivation}
\end{table*}

==> Tables/policies.tex <==
\begin{table}[h!]
\centering
\caption{\xy{Just an example of the format.}}
\resizebox{1\linewidth}{!}{
\begin{threeparttable}{
\begin{tabular}{cccc}
\toprule[1.2pt]
\textbf{Store name} & \textbf{Privacy policy} & \textbf{Usage guidelines} & \textbf{Terms of service} \\ \midrule
GPT Store    & \yes & \yes & \yes \\ 
FlowGPT      & \partialcell & \partialcell & \yes \\ 
Poe          & \yes & \yes & \yes \\ 
Coze         & \yes & \no & \yes \\ 
Cici         & \yes & \no & \yes \\ 
Character.AI & \yes & \partialcell & \yes \\ 
\bottomrule[1.2pt]
\end{tabular}}
\begin{tablenotes}
    \footnotesize
    \item \yes\ indicates detailed policy, \partialcell\ indicates incomplete policy, \no\ indicates the absence of policy.
\end{tablenotes}
\end{threeparttable}}
\label{tab:policy}
\end{table}

==> Tables/result_old.tex <==
\begin{table*}[!htbp]
    \centering
    \caption{Overview of numbers of cloning and squatting apps in six LLM app stores.}
    \resizebox{0.9\linewidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{lrrrrrr}
        \toprule[1.2pt]
        \textbf{Store} & \textbf{\# LLM apps} & \textbf{\makecell{ident\_inst\tnote{1} \\ (\% of total)}} & \textbf{\makecell{ident\_desc\tnote{2} \\ (\% of total)}} & \textbf{\makecell{ident\_both\tnote{3} \\ (\% of total)}} & 
        \textbf{\makecell{95\_sim\_inst\tnote{4} \\ (\% of total)}} & 
        \textbf{\makecell{95\_sim\_sem\tnote{5} \\ (\% of total)}} \\
        \midrule
        GPT Store      & 662,294               & 36 (0.005\%)               & 7,570 (1.14\%)             & 0                       & 22 (0.003\%)               & 92 (0.014\%)              \\
        FlowGPT        & 34,271                & 784 (2.29\%)               & 944 (2.75\%)               & 121 (0.35\%)            & 1,396 (4.07\%)             & 1,705 (4.98\%)            \\
        Poe            & 16,544                & 185 (1.12\%)               & 210 (1.27\%)               & 76 (0.46\%)             & 188 (1.14\%)               & 258 (1.56\%)              \\
        Coze           & 51,912                & 33 (0.06\%)                & 0                         & 0                       & 23 (0.04\%)                & 8 (0.01\%)                \\
        Cici           & 13,060                & 1 (0.01\%)                 & 1 (0.01\%)                & 0                       & 0                         & 0                         \\
        Character.AI   & 7,048                 & 20 (0.28\%)                & 40 (0.57\%)               & 12 (0.17\%)             & 13 (0.18\%)                & 50 (0.71\%)               \\
        \midrule
        Total & 785,129      & 1,058 (0.13\%)     & 8,765 (1.12\%)    & 209 (0.03\%)    & 1,637 (0.21\%)     & 2,113 (0.27\%)    \\
        \bottomrule[1.2pt]
    \end{tabular}
    \begin{tablenotes}  % 开始 tablenotes 环境，添加对应的脚注内容
        \footnotesize
        \item[1] ident\_inst: Number of apps with identical instructions.
        \item[2] ident\_desc: Number of apps with identical descriptions.
        \item[3] ident\_both: Number of apps with both identical instructions and descriptions.
        \item[4] 95\_sim\_inst: Apps with 95\%+ similarity in instructions.
        \item[5] 95\_sim\_sem: Apps with 95\%+ semantic similarity.
    \end{tablenotes}
    \end{threeparttable} 
    }
    \label{tab:data-summary}
\end{table*}


==> Tables/six-platforms.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Six LLM app stores from which we collect information.}
    \resizebox{1\linewidth}{!}{\begin{tabular}{lrrrrrr}
        \toprule[1.2pt]
        \textbf{Platform} & \textbf{Website} \\
        \midrule
        GPT Store & https://chatgpt.com/gpts \\
        FlowGPT & https://flowgpt.com/ \\
        Poe & https://poe.com \\
        Coze & https://www.coze.com \\
        Cici & https://www.ciciai.com/chat/ \\
        Charcter.Al & https://character.ai/ \\
        \bottomrule[1.2pt]
    \end{tabular}}
    \label{tab:six-platforms}
\end{table}


==> Tables/top-10-gpts.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Top 10 Apps from GPT Store.}
    \resizebox{1\linewidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{lrrrrrr}
        \toprule[1.2pt]
        \textbf{App Name} & \textbf{Author Name} & \textbf{Conversation Count} \\
        \midrule
        image generator     & NAIF J ALOTAIBI       & 6M+  \\ 
        Consensus           & consensus.app         & 5M+  \\
        Write For Me        & puzzle.today          & 4M+ \\
        Logo Creator        & None                 & 2M+  \\
        Canva               & canva.com            & 2M+ \\
        Scholar GPT         & awesomegpts.ai        & 2M+ \\
        Code Copilot        & promptspellsmith.com  & 2M+ \\
        Cartoonize Yourself & karenxcheng.com      & 2M+ \\
        Diagrams\tnote{1}   & helpful.dev            & 1M+ \\
        Python              & Nicholas Barker        & 1M+ \\
        \bottomrule[1.2pt]
    
    \end{tabular}
    \begin{tablenotes}  % 开始 tablenotes 环境，添加对应的脚注内容
        \footnotesize
        \item[1] Diagrams: The full name of this app is ``Diagrams: Show Me | charts, presentations, code''.
    \end{tablenotes}
    \end{threeparttable} }
    \label{tab:top10-GPTs}
\end{table}

==> Tables/top5-author.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Top 5 authors with the highest number of applications.}
    \resizebox{1\linewidth}{!}{\begin{tabular}{lrrrrrr}
        \toprule[1.2pt]
        \textbf{Author Name} & \textbf{Top 1 App of the Author} & \textbf{Duplicate Count} \\
        \midrule
        ai-gen.co & News & 3633 \\
        hix.ai & AI Humanizer \& Paraphraser & 335 \\
        Internethandel & Generador de Imágenes & 316 \\
        Kenneth Bastian &  Data Analysis \& Report AI & 283 \\
        Josh Brent N. Villocido & Books & 172 \\
        \bottomrule[1.2pt]
    \end{tabular}}
    \label{tab:author-name-top5}
\end{table}

